TuneTables: Context Optimization for Scalable Prior-Data Fitted Networks

While tabular classification has traditionally relied on from-scratch training, a recent breakthrough called prior-data fitted networks (PFNs) challenges this approach. Similar to large language models, PFNs make use of pretraining and in-context learning to achieve strong performance on new tasks in a single forward pass. However, current PFNs have limitations that prohibit their widespread adoption. Notably, TabPFN achieves very strong performance on small tabular datasets but is not designed to make predictions for datasets of size larger than 1000. In this work, we overcome these limitations and substantially improve the performance of PFNs via context optimization. We introduce TuneTables, a parameter-efficient fine-tuning strategy for PFNs that compresses large datasets into a smaller learned context. We conduct extensive experiments on 19 algorithms over 98 datasets and find that TuneTables achieves the best performance on average, outperforming boosted trees such as CatBoost, while optimizing fewer than 5% of TabPFN's parameters. Furthermore, we show that TuneTables can be used as an interpretability tool and can even be used to mitigate biases by optimizing a fairness objective. We open-source our code and raw results at https://github.com/penfever/TuneTables.

==> algorithms/tt_alg.tex <==
\caption{Optimized Model Selection and Feature Selection Algorithm. FeatSS wraps standard feature subselection algorithms as described in \cref{sec:background}. ZeroPad pads the number of features to exactly 100, following \cite{hollmann2022tabpfn}. Model variant $ZS$ is the standard TabPFN model of \cite{hollmann2022tabpfn}. $PT+DEC$ co-trains prompt and decoder layer, as described in \cref{subsec:extended_classes}. $PT+ENS$ refers to prompt tuning with ensembling, described in \cref{app:pt-experiments}. $CT$ and $NCT$ settings are also defined in \cref{app:pt-experiments}.}
\begin{algorithmic}[1]
\REQUIRE dataset $D$, model variants $ZS$, $PT+ENS$, $PT+DEC$, sample cutoff $k$, feature cutoff $j$, class cutoff $l$, maximum runtime $t$, feature selection algorithm list $fs$, HPO search space $hl$, optimization objective list $o$
\STATE $search\_space \gets [\text{hparams} = hl, \text{models} = [], \text{feature\_subsel} = []]$
\STATE $d_f \gets \# \text{features of } D$
\STATE $d_c \gets \# \text{classes of } D$
\STATE $d_n \gets \# \text{samples of } D$
\IF{$d_f > j$}
    \STATE $feature\_subsel \gets [\text{FeatSS}(j, d_f, \text{alg}) \text{ for alg in } fs]$
\ELSIF{$d_f < j$}
    \STATE $feature\_subsel \gets [\text{ZeroPad}(j, d_f)]$
\ELSE
    \STATE $feature\_subsel \gets [\text{Identity}()]$
\ENDIF
\IF{$d_c > l$}
    \STATE $models \gets [PT+DEC(D)]$
\ELSIF{$d_n < k$}
    \STATE $models \gets [ZS(D[:k])]$
\ELSE
    \STATE $models \gets [ZS(D[:k]), PT+ENS(D, CT), PT+ENS(D, NCT)]$
\ENDIF
\RETURN $\text{FitAndGridSearch}(D, o, search\_space, t)$
\end{algorithmic}
\label{alg:tt_main}

==> algorithms/tt_gridsearch.tex <==
\caption{Fit and Grid Search Algorithm}
\begin{algorithmic}[1]
\REQUIRE Labeled dataset $D$, optimization objectives $o$, search space $search\_space$ (list of lists of hyperparameters, models, and feature subselection methods), maximum search time $t$
\ENSURE Explored spaces and outputs
\STATE $explored\_spaces \gets []$
\STATE $outputs \gets []$
\STATE $i \gets 0$
\WHILE{$i < t$}
    \STATE $next\_space \gets \text{select without replacement a new combination from } search\_space$
    \STATE $start \gets \text{CurrentTime()}$
    \STATE $outputs \gets \text{Model}(D, \text{HParams}, \text{Features})$
    \STATE $explored\_spaces \gets next\_space$
    \STATE $i \gets i + (\text{CurrentTime()} - start)$
\ENDWHILE
\STATE $b, idx\_b \gets 0, -1$
\FOR{$out, idx\_out \text{in Enum(outputs)}$}
    \FOR{$obj$ in $o$}
        \IF{$obj > b$}
            \STATE $b \gets obj$
            \STATE $idx\_b \gets idx\_out$
        \ENDIF
    \ENDFOR
\ENDFOR
\RETURN $explored\_spaces[idx\_b], outputs[idx\_b]$
\end{algorithmic}
\label{alg:tt_gridsearch}
